Combinatorial Auctions with Interdependent Valuations: SOS to the Rescue

We study combinatorial auctions with interdependent valuations. In such settings, each agent $i$ has a private signal $s_i$ that captures her private information, and the valuation function of every agent depends on the entire signal profile, ${\bf s}=(s_1,\ldots,s_n)$. The literature in economics shows that the interdependent model gives rise to strong impossibility results, and identifies assumptions under which optimal solutions can be attained. The computer science literature provides approximation results for simple single-parameter settings (mostly single item auctions, or matroid feasibility constraints). Both bodies of literature focus largely on valuations satisfying a technical condition termed {\em single crossing} (or variants thereof). We consider the class of {\em submodular over signals} (SOS) valuations (without imposing any single-crossing type assumption), and provide the first welfare approximation guarantees for multi-dimensional combinatorial auctions, achieved by universally ex-post IC-IR mechanisms. Our main results are: $(i)$ 4-approximation for any single-parameter downward-closed setting with single-dimensional signals and SOS valuations; $(ii)$ 4-approximation for any combinatorial auction with multi-dimensional signals and {\em separable}-SOS valuations; and $(iii)$ $(k+3)$- and $(2\log(k)+4)$-approximation for any combinatorial auction with single-dimensional signals, with $k$-sized signal space, for SOS and strong-SOS valuations, respectively. All of our results extend to a parameterized version of SOS, $d$-SOS, while losing a factor that depends on $d$.

==> noexpost.tex <==
\section{Proof of Lower Bound Theorem \ref{thm:noexpost}}\label{sec:noexpost}

\noindent{\bf Theorem \ref{thm:noexpost}}:

No ex-post IC-IR mechanism (not necessarily universal) for selling a single item can get a better approximation than
	\begin{enumerate}
		\item [(a)] a factor of 2 for SOS valuations.
		\item [(b)] a factor of $\Omega(\sqrt{d})$ for $d$-SOS valuations.
	\end{enumerate}

\begin{proof}
	Let $x_i(\mathbf{s})$ be the probability agent $i$ is allocated at signal profile $\mathbf{s}$. Notice that for every $\mathbf{s}$, $\sum_i x_i(\mathbf{s})\leq 1$, otherwise the allocation rule is not feasible.
	\begin{enumerate}
		\item [(a)] Consider the case where there are two agents, 1 and 2, $s_1\in\{0,1\}$ and agent~2 has no signal. The valuations are $v_1(0)=1$, $v_1(1)=1+\epsilon$, $v_2(0)=0$ and $v_2(1)=H$ for $H\gg 1\gg \epsilon$. It is easy to see the valuations are SOS.
		
		 In order to get better than a 2-approximation at $s_1 = 0$, we must have $x_1(0)>1/2$.  By monotonicity, this forces $x_1(1)>1/2$ as well, and hence $x_2(1)<1/2$ by feasibility. This implies that the expected welfare when $s_1=1$ is $x_1(1)v_1(1)+x_2(1)v_2(1) < H/2+1$, while the optimal welfare when $s_1 = 1$ is $H$. For a large $H$, this approaches a 2-approximation.  Note that this lower bound applies even given a known prior distribution on the signals in the event that we have a prior on the signals that satisfies: $\Pr[s_1=0]\cdot 1=\Pr[s_1=1]\cdot H$.
		\item [(b)] Consider the case where there are $n=\sqrt{d}$ agents and $s_i\in \{0,1\}$ for every agent $i$. The valuation of agent $i$ is
		\begin{eqnarray*}
			v_i(\mathbf{s})=\begin{cases}
				\sum_{j\neq i} s_j +\epsilon\cdot s_i\quad &\exists j\neq i\ :\ s_j =0\\
				d +\epsilon\cdot s_i\quad &s_j=1 \ \forall j\neq i,
			\end{cases}
		\end{eqnarray*}
		where $\epsilon\rightarrow 0$.
		
		To see that the valuations are $d$-SOS, notice that whenever a signal $s_j$ changes from~0 to~1, the valuation of agent $i\neq j$ increases by~1 \textit{unless} all other signals beside $i$'s are already set to $1$, in which case the valuation increases by $d-\sqrt{d}+2 < d$.
		Consider valuation profiles $\mathbf{s^i}=(0_i, \mathbf{1}_{-i})$. Note that by monotonicity, for every truthful mechanism, it must be the case that $x_i(\mathbf{s^i})\leq x_i(\mathbf{1})$. Since any feasible allocation rule must satisfy $\sum_{i=1}^{\sqrt{d}}x_i(\mathbf{1})\leq 1$, then it must be the case there exists some agent $i$ such that $x_i(\mathbf{1})\leq \frac{1}{\sqrt{d}}$, which by monotonicity implies that $x_i(\mathbf{s^i})\leq \frac{1}{\sqrt{d}}$. However, at profile $\mathbf{s^i}$, $v_i(\mathbf{s^i})=d$ while $v_j(\mathbf{s^i})=\sqrt{d}-2< \sqrt{d}$ for all $j\neq i$, so we get that the expected welfare of the mechanism at $\mathbf{s^i}$ is at most $x_i(\mathbf{s^i})\cdot d + (1-x_i(\mathbf{s^i}))\cdot \sqrt{d} \leq 2\sqrt{d},$ while the optimal welfare is $d$. Again, the lower bound also applies to the setting with known priors on the signals using a prior that satisfies: $\Pr[\mathbf{s^i}]=\Pr[\mathbf{s^j}]=\frac{1}{\sqrt{d}}$ for all $i$ and $j$.
	\end{enumerate}
\end{proof}


==> notations.tex <==
%general machinery

%% General machinery
\newcommand{\AutoAdjust}[3]{\mathchoice{ \left #1 #2  \right #3}{#1 #2 #3}{#1 #2 #3}{#1 #2 #3} }
\newcommand{\Xcomment}[1]{{}}
\newcommand{\eval}[1]{\left.#1\vphantom{\big|}\right|}
\newcommand{\inteval}[1]{\Big[#1\Big]}
\newcommand{\InParentheses}[1]{\AutoAdjust{(}{#1}{)}}
\newcommand{\InBrackets}[1]{\AutoAdjust{[}{#1}{]}}% {\left[{#1}\right]}
%\newcommand{\Ex}[2][]{\operatorname{\mathbf E}_{_{#1}}\InBrackets{#2}}
\newcommand{\Ex}[2][]{\operatorname{\mathbf E}_{#1}\InBrackets{#2\vphantom{E_{F}}}}
\newcommand{\Exlong}[2][]{\operatornamewithlimits{\mathbf E}\limits_{#1}\InBrackets{#2\vphantom{\operatornamewithlimits{\mathbf E}\limits_{#1}}}}
\newcommand{\Prx}[2][]{\operatorname{\mathbf{Pr}}_{#1}\InBrackets{#2}}
\newcommand{\Prlong}[2][]{\operatornamewithlimits{\mathbf Pr}\limits_{#1}\InBrackets{#2\vphantom{\operatornamewithlimits{\mathbf Pr}\limits_{#1}}}}
\def\prob{\Prx}
\def\expect{\Ex}
\newcommand{\super}[1]{^{(#1)}}
\newcommand{\dd}{\mathrm{d}}  % for integrals
\newcommand{\given}{\;\mid\;}



\newcommand{\Ell}{\ensuremath{\mathcal{L}}}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\vr}[1]{{\mathbf{#1}}}
\newcommand{\bydef}{\stackrel{\bigtriangleup}{=}}
\newcommand{\eps}{\varepsilon}
%\newcommand{\qed}}{\hfill$\bf{\Box}$}
\newcommand{\mm}[1]{\mathrm{#1}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mb}[1]{\mathbf{#1}}
\newcommand{\vect}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\R}{\mathbb{R}}

\def \EE   {{\mathbb E}}
\def \OPT {\mathcal{OPT}}
\def \vf  {\textrm{vf}}
\def \dvf {\varphi}
\def \utility {u}
\def \reals {{\mathbb R}}

\newcommand{\Idr}[1]{\mathds{1}\InBrackets{#1\vphantom{\sum}}}

%Probability notations

\newcommand{\dist}{\mathcal{F}}
\newcommand{\disti}[1][i]{{\mathcal{F}_{#1}}}
\newcommand{\distsmi}[1][i]{\dists_{\text{-}#1}}
\newcommand{\dists}{\vect{\dist}}
\newcommand{\distw}{\widetilde{\mathcal{F}}}

\newcommand{\valdist}{\mathcal{F}}
\newcommand{\valdists}{\vect{\valdist}}
\newcommand{\valdisti}[1][i]{{\valdist_{#1}}}
\newcommand{\valdistsmi}[1][i]{\valdists_{\text{-}#1}}


\newcommand{\dens}{f}
\newcommand{\denss}{\vect{ \dens}}
\newcommand{\densi}[1][i]{{\dens_{#1}}}

%Combinatorial description
\newcommand{\agents}{N}
\newcommand{\nagent}{n}
\newcommand{\goods}{M}
\newcommand{\nitem}{m}
\newcommand{\auction}{A}

\newcommand{\weight}{w}
\newcommand{\partition}{\Gamma}
\newcommand{\partitioni}{\Gamma_i}

\newcommand{\CWE}[0]{\textsf{CWE}}
\newcommand{\ef}[0]{envy free}
\newcommand{\EF}[0]{EF}
\newcommand{\CWEWOMC}[0]{CWE without market clearance}
\newcommand{\SW}[0]{\textsf{SW}}
\newcommand{\Revenue}[0]{\textsf{Rev}}

%Game theory notations
\newcommand{\bid}{b}
\newcommand{\bids}{\vect{\bid}}
\newcommand{\bidsmi}[1][i]{\bids_{\text{-}#1}}
\newcommand{\bidi}[1][i]{{\bid_{#1}}}

\newcommand{\val}{v}
\newcommand{\vals}{\vect{\val}}
\newcommand{\valsmi}[1][i]{\vals_{\text{-}#1}}
\newcommand{\vali}[1][i]{{\val_{#1}}}
\newcommand{\valith}[1][i]{{\val_{(#1)}}}

\newcommand{\wal}{\widetilde{v}}
\newcommand{\wals}{\vect{\wal}}
\newcommand{\walsmi}[1][i]{\wals_{\text{-}#1}}
\newcommand{\wali}[1][i]{{\wal_{#1}}}



\newcommand{\util}{u}
\newcommand{\utils}{\vect{\util}}
\newcommand{\utili}[1][i]{\util_{#1}}
\newcommand{\utilsmi}[1]{\utils_{\text{-}#1}}



\newcommand{\price}{p}
\newcommand{\prices}{\vect{\price}}
\newcommand{\pricei}[1][i]{{\price_{#1}}}

\newcommand{\payment}{\rho}
\newcommand{\payments}{\vect{\payment}}
\newcommand{\paymenti}[1][i]{{\payment_{#1}}}


\newcommand{\type}{t}
\newcommand{\types}{\vect{\type}}
\newcommand{\typei}[1][i]{{\type_{#1}}}
\newcommand{\typesmi}[1][i]{\types_{\text{-}#1}}

\newcommand{\alloc}{X}
\newcommand{\allocs}{\vect{\alloc}}
\newcommand{\allocsmi}[1][i]{\allocs_{\text{-}#1}}
\newcommand{\alloci}[1][i]{{\alloc_{#1}}}

\newcommand{\opt}{\text{OPT}}
\newcommand{\opts}{\vect{ \opt}}
\newcommand{\opti}[1][i]{{\opt_{#1}}}
\newcommand{\optsmi}[1][i]{\opts_{\text{-}#1}}




\newcommand{\talloc}{Y}
\newcommand{\tallocs}{\vect{\talloc}}
\newcommand{\talloci}[1][i]{{\talloc_{#1}}}
\newcommand{\tallocsmi}[1][i]{\tallocs_{\text{-}#1}}

\newcommand{\rank}{r}
\newcommand{\ranks}{\vect{\rank}}
\newcommand{\ranki}[1][i]{{\rank_{#1}}}
\newcommand{\ranksmi}[1][i]{\ranks_{\text{-}#1}}

\newcommand{\crit}{\theta}
\newcommand{\crits}{\vect{\crit}}
\newcommand{\criti}[1][i]{{\crit_{#1}}}
\newcommand{\critsmi}[1][i]{\crits_{\text{-}#1}}

\newcommand{\decl}{d}
\newcommand{\decls}{\vect{\decl}}
\newcommand{\decli}[1][i]{{\decl_{#1}}}
\newcommand{\declsmi}[1][i]{\decls_{\text{-}#1}}

\newcommand{\demand}{D}
\newcommand{\demands}{\vect{\demand}}
\newcommand{\demandi}[1][i]{{\demand_{#1}}}
\newcommand{\demandsmi}[1][i]{\demands_{\text{-}#1}}

\newcommand{\sold}{{\texttt{SOLD}}}
\newcommand{\soldi}[1][i]{\sold_{#1}}


%algorithm
\newcommand{\CWEalg}{{\sc CWE} algorithm}
%\newcommand{\pool}{\text{Pool}}

\newcommand{\Pool}{\text{Pool}}
\newcommand{\Pop}{\textbf{Pop}}
\newcommand{\Push}{\textbf{Push}}
\newcommand{\Bundle}{\textbf{Bundle}}
\newcommand{\ResolveConflict}{\textbf{ResolveConflict}}



%algorithm poly-time

\newcommand{\Reject}{\text{Reject}}
\newcommand{\AllocateDemand}{\textbf{AllocateDemand}}
\newcommand{\RaisePrices}{\textbf{RaisePrices}}





==> old-separable.tex <==
In what follows, we consider the case where every agent $i$ has a signal that is composed of a real number for every set $T \subseteq [m]$; i.e., $s_i = \{s_{iT}\}_{T \subseteq [m]}$.
The valuation of agent $i$ for a set $T$ is some function of the signals of all the agents for $T$;
i.e., $v_{iT} = v_{iT}(s_{1T}, \ldots, s_{nT})$.
(The model considered in [JM'00] can be handled in a similar manner, we choose this model for simplicity of presentation).

The submodularity condition is the following:
$$\forall k, T, \vec{s}_{-i} \leq \vec{s'}_{-i} \quad \quad \frac{\partial}{\partial s_i} v_{kT}(s_i, \vec{s}_{-i}) \geq \frac{\partial}{\partial s_i} v_{kT}(s_i, \vec{s'}_{-i}).$$

We assume that values are {\em separable}; this means that for every agent $i$ and bundle $T$ it holds that
$$v_{iT}(s) = g_{iT}(s_{-i}) + f_{iT}(s_i),$$
for some submodular function $g_{iT}$ and a monotone function $f_{iT}$.

\paragraph{The mechanism.}
The mechanism partitions the bidders (independently) into sets $A$ and $B$ uniformly at random.
Let $s_{AT}$ denote the vector of signals $s_{jT}$ for all agents $j \in A$.
%For every agent $i \in B$ and every bundle $T \subseteq [m]$, let $w_{iT}(s) = v_{iT}(s_{iT}, \vec{s}_{AT}, \vec{0}_{B_{-i}})$.
%For every agent $i \in B$ and every bundle $T \subseteq [m]$, let $w_{iT}(s) = 0$.

For every agent $i$ and bundle $T \subseteq [m]$, let
$$
w_{iT}(s)=
\begin{cases}
  v_{iT}(s_{iT}, \vec{s}_{AT}, \vec{0}_{B_{-i}}), & \mbox{if $i\in B$} \\
  0, & \mbox{otherwise}.
\end{cases}
$$

The allocation rule:
Allocate according to the allocation that maximizes the social welfare based on the $w$'s rather than the real values $v$'s.
I.e., given a vector of reported signals $s$, return
$$T = \argmax_{R=(R_1,\ldots,R_n)} \sum_{i=1}^{n} w_{iR_i}(s).$$

The payment rule (this resembles the VCG payment rule for independent private values):
%$$p_{i}(s) = v_{i T_i}(\vec{0}_A, 0_i, \vec{s}_{B_{-i}}) - v_{iT_i}(\vec{0}) + \opt^{-i}\left(\{v_j(s_j, \vec{s}_A, \vec{0}_{B_{-j}})\} _{j \neq i \in B}\right) - \sum _{j \neq i \in B} v_{j T_j}(s_j, \vec{s}_A, \vec{0}_{B_{-j}}).$$

*** UP TO HERE ***

==> separable.tex <==
In what follows, we consider the case where every agent $i$ has a signal that is composed of a real number for every set $T \subseteq [m]$; i.e., $s_i = \{s_iT\}_{T \subseteq [m]}$.
The valuation of agent $i$ for a set $T$ is some function of the signals of all the agents for $T$; 
i.e., $v_{iT} = v_{iT}(s_1T, \ldots, s_nT)$.
(The model considered in [JM'00] can be handled in a similar manner, we choose this model for simplicity of presentation).

The submodularity condition is the following: 
$$\forall k, T \quad \quad \vec{s}_{-i} \leq \vec{s'}_{-i} \quad \quad \frac{\partial}{\partial s_i} v_{kT}(s_i, \vec{s}_{-i}) \geq \frac{\partial}{\partial s_i} v_{kT}(s_i, \vec{s'}_{-i}).$$

We assume that values are {\em separable}; this means that for every agent $i$ and bundle $T$ it holds that
$$v_{iT}(s) = g_{iT}(s_{-i}) + f_{iT}(s_i),$$
for some submodular function $g_{iT}$ and a monotone function $f_{iT}$.

\paragraph{The mechanism.}
The mechanism partitions the bidders into sets $A$ and $B$ uniformly and independently at random.
Let $s_{AT}$ denote the vector of signals $s_{jT}$ for all agents $j \in T$.
For every agent $i \in B$ and every bundle $T \subseteq [m]$, let $w_{iT}(s) = v_{iT}(s_{iT}, \vec{s}_{AT}, \vec{0}_{B_{-i}})$.
For every agent $i \in B$ and every bundle $T \subseteq [m]$, let $w_{iT}(s) = 0$.

The allocation rule: 
Allocate according to the allocation that maximizes the social welfare based on the $w$'s rather than the real values $v$'s.
I.e., given a vector $s$ of reports, return $T = \argmax_{R=(R_1,\ldots,R_n)} $\sum_{i=1}^{n} w_{iR_i}(s)$. 

The payment rule (this resembles the VCG payment rule for independent private values): 
$$p_{i}(s) = v_{i T_i}(\vec{0}_A, 0_i, \vec{s}_{B_{-i}}) - v_{iT_i}(\vec{0}) + \opt^{-i}\left(\{v_j(s_j, \vec{s}_A, \vec{0}_{B_{-j}})\} _{j \neq i \in B}\right) - \sum _{j \neq i \in B} v_{j T_j}(s_j, \vec{s}_A, \vec{0}_{B_{-j}}).$$

*** UP TO HERE ***



==> ssoslogk.tex <==
\section{$O(\log k)$-Approximation with Strong-SOS Valuations} \label{sec:k-sig-ssm}
Strong-SOS valuations let us use a bucketing technique in order to give an $O(\log k)$-approximation % $O(d^2\log k)$ approximation
to the \textsf{SELF} component in the decomposition depicted by Equation~\eqref{eq:decomposition}. Consider the \textsf{SELF} term in Equation~\eqref{eq:decomposition}. We can bound this term as follows:
\begin{comment}
\begin{eqnarray}
	\mathsf{SELF} &=&	\sum_{\ell=1}^{k-1}\sum_{i\ :\  s_i=\ell}d\cdot v_{iT_i^*}(\mathbf{0}_{-i}, s_i)\nonumber\\
	 & = & \sum_{\ell=1}^{\log_2 k}\sum_{i\ :\ 2^{\ell-1}\leq s_i < 2^\ell} d\cdot v_{iT_i^*}(\mathbf{0}_{-i}, s_i)\nonumber\\
	 & \leq & \sum_{\ell=1}^{\log_2 k}\sum_{i\ :\ 2^{\ell-1}\leq s_i < 2^\ell} d(d+1)\cdot v_{iT_i^*}(\mathbf{0}_{-i}, 2^{\ell-1}), \label{eq:selfbound_strong_submod}
\end{eqnarray}
where the inequality follows the definition of $d$-strong-submodularity.
\end{comment}
\begin{eqnarray}
\mathsf{SELF} &=&	\sum_{\ell=1}^{k-1}\sum_{i\ :\  s_i=\ell}v_{iT_i^*}(\mathbf{0}_{-i}, s_i)\nonumber\\
& = & \sum_{\ell=1}^{\log_2 k}\sum_{i\ :\ 2^{\ell-1}\leq s_i < 2^\ell} v_{iT_i^*}(\mathbf{0}_{-i}, s_i)\nonumber\\
& \leq & \sum_{\ell=1}^{\log_2 k}\sum_{i\ :\ 2^{\ell-1}\leq s_i < 2^\ell} v_{iT_i^*}(\mathbf{0}_{-i}, 2^{\ell-1}), \label{eq:selfbound_strong_submod}
\end{eqnarray}
where the inequality follows the definition of strong-SOS valuations.

We introduce mechanism \texttt{Random Bucket} to give an $O(\log k)$-approximation
%$O(d^2\log k)$
to the upper bound in Equation~\eqref{eq:selfbound_strong_submod}.

\vspace{0.1in}
\noindent Mechanism \texttt{Random Bucket}:
\begin{itemize}
	\item choose $\ell$ uniformly in $\{1,\ldots, \log_2 k\}$.
	\item Let $N_{B_\ell}=\{i\ :\ \mbox{such that }s_i\geq 2^{\ell-1}\}$ be the agents with signal at least $2^{\ell-1}$ and $N_{\neg B_\ell}=[n]\setminus N_{B_\ell}$.
	\item For $i\in N_{B_\ell}$ and bundle $T$, let $\bar{v}_{iT}:=v_{iT}(\mathbf{s}_{N_{\neg B_\ell}},\mathbf{2^{\ell-1}}_{N_{B_\ell}})$ (and $\bar{v}_{iT}:=0$ for $i\in N_{\neg B_\ell}$).
	\item Let the allocation be $$\bar{T} \in \argmax_{S=\{S_i\}_{i\in N_{B_\ell}}} \sum_{i\in N_{B_\ell}}\bar{v}_{iS_i}.$$ (\textit{i.e.}, the allocation that maximizes the ``welfare'' of high agents using values $\bar{v}_{iT}$.)
	%\item Compute the optimal allocation $$\bar{T}=\{\bar{T}_i\}_{i\in N_{B_\ell}}$$ for agents in $N_{B_\ell}$ using values $\bar{v}_{iT}$.
	\item Agent $i$ that receives bundle $\bar{T}_i$ pays $v_{i\bar{T}_i}(\mathbf{s}_{-i}, s_i=2^{\ell-1}-1)$.
\end{itemize}

We show the following approximation guarantee regarding \texttt{Random Bucket}.
\begin{comment}
\begin{lemma} \label{lem:self_cover_strongly_submod}
	For $d$-strongly-submodular valuations, the \texttt{Random Threshold} mechanism is truthfulness and gives a $d(d+1)\log_2{k}$ approximation to the \textsf{SELF} component of the optimal social welfare.
\end{lemma}	
\begin{proof}
	The proof of truthfulness is identical to that of mechanism \texttt{Random Threshold}, as both are threshold based mechanisms. The proof of the approximation guarantee is also very similar to that of \texttt{Random Threshold}.
	
	 Consider a threshold $2^{\ell-1}$ for $\ell\in \{1,\ldots,k-1\}$ chosen in \texttt{Random Bucket}. Whenever $\ell$ is chosen, we have that
	 \begin{eqnarray*}
	 	\sum_{i\ :\ 2^{\ell-1}\leq s_i < 2^\ell} \bar{v}_{iT_i^*}  \ = \  \sum_{i\ :\ 2^{\ell-1}\leq s_i < 2^\ell} v_{iT_i^*}(\mathbf{s}_{N_{\neg B_\ell}}	,\mathbf{2^{\ell-1}}_{N_{B_\ell}}) \ \geq\ \sum_{i\ :\ 2^{\ell-1}\leq s_i < 2^\ell} v_{iT_i^*}(\mathbf{0}_{-i},2^{\ell-1}).
	 \end{eqnarray*}
	 Since \texttt{Random Bucket} chooses an allocation that maximizes the $\bar{v}_{iT}$'s, the value of the allocation is only larger. Because $v_{i\bar{T}_i}(\mathbf{s})\geq \bar{v}_{i\bar{T}_i}$, we get that if $\ell$ was chosen, which happens with probability $\frac{1}{\log_2{k}}$, the welfare achieved is at least $\sum\limits_{i\ :\ 2^{\ell-1}\leq s_i < 2^\ell} v_{iT_i^*}(\mathbf{0}_{-i},s_i).$ Therefore, the welfare from running \texttt{Random Bucket} is at least
	 $$\sum_{\ell=1}^{\log_2{k}} \frac{1}{\log_2{k}}\sum_{i\ :\ 2^{\ell-1}\leq s_i < 2^\ell} v_{iT_i^*}(\mathbf{0}_{-i},s_i),\geq \frac{\mathsf{SELF}}{d(d+1)\log_2{k}}.$$
	
\end{proof}
\end{comment}

\begin{lemma} \label{lem:self_cover_strongly_submod}
	For strong-SOS valuations, the \texttt{Random Bucket} mechanism is ex-post IC-IR and gives a $2\log_2{k}$ approximation to the \textsf{SELF} component of the optimal social welfare.
\end{lemma}	
\begin{proof}
	The proof of ex-post IC-IR is identical to that of mechanism \texttt{Random Threshold}, as both are threshold-based mechanisms. The proof of the approximation guarantee is also very similar to that of \texttt{Random Threshold}.
	
	Consider a threshold $2^{\ell-1}$ for $\ell\in \{1,\ldots,k-1\}$ chosen in \texttt{Random Bucket}. Whenever $\ell$ is chosen, we have that
	\begin{eqnarray*}
		\sum_{i\ :\ 2^{\ell-1}\leq s_i < 2^\ell} \bar{v}_{iT_i^*}  \ = \  \sum_{i\ :\ 2^{\ell-1}\leq s_i < 2^\ell} v_{iT_i^*}(\mathbf{s}_{N_{\neg B_\ell}}	,\mathbf{2^{\ell-1}}_{N_{B_\ell}}) \ \geq\ \sum_{i\ :\ 2^{\ell-1}\leq s_i < 2^\ell} v_{iT_i^*}(\mathbf{0}_{-i},2^{\ell-1}).
	\end{eqnarray*}
	Since \texttt{Random Bucket} chooses an allocation that maximizes the $\bar{v}_{iT}$'s, the value of the allocation is only larger. Because $v_{i\bar{T}_i}(\mathbf{s})\geq \bar{v}_{i\bar{T}_i}$, we get that if $\ell$ was chosen, which happens with probability $\frac{1}{\log_2{k}}$, the welfare achieved is at least $\sum\limits_{i\ :\ 2^{\ell-1}\leq s_i < 2^\ell} v_{iT_i^*}(\mathbf{0}_{-i},s_i).$ Therefore, the welfare from running \texttt{Random Bucket} is at least
	$$\sum_{\ell=1}^{\log_2{k}} \frac{1}{\log_2{k}}\sum_{i\ :\ 2^{\ell-1}\leq s_i < 2^\ell} v_{iT_i^*}(\mathbf{0}_{-i},s_i),\geq \frac{\mathsf{SELF}}{2\log_2{k}}.$$
	
\end{proof}


Mechanism \texttt{$k$-signals Strong-SOS} (\texttt{$k$-SS}) runs \texttt{Random Bucket} with probability $p_{RB}=\frac{log_2{k}}{log_2{k}+2}$ %\frac{d\log_2{k}}{d\log_2{k}+2}$
and mechanism \texttt{Random Sampling} with probability $1-p_{RB}$.

\begin{theorem}	\label{thm:k-sig-ssm}
	For every combinatorial auction with single-dimensional signals with strong-SOS valuations and signal space of size $k$, i.e. $s_i \in \{0, 1,\ldots, k-1\} \, \forall i$, mechanism \texttt{$k$-SS} is ex-post IC-IR, and gives $(2\log_2{k}+4)$-approximation to the optimal social welfare.
	%More generally, for $d$-strongly-submodular valuations we get $(d(d+1)\log_2{k}+2(d+1))$-approximation.
\end{theorem}
\begin{proof}
	We already established that both \texttt{Random Bucket} and \texttt{Random Sampling} are ex-post IC-IR, hence  \texttt{$k$-SS} is ex-post IC-IR as well. As for the approximation, according to Lemma~\ref{lem:self_cover_strongly_submod}, with probability $p_{RB}$ we get $2\log_2{k}$-approximation %$d(d+1)\log_2{k}$ approximation
	to \textsf{SELF}, and according to Lemma~\ref{lem:other_cover}, with probability $1-p_{RB}$ we get a $4$-approximation % $2(d+1)$ approximation
	to \textsf{OTHER}. Overall, the expected welfare is at least
\begin{comment}
	\begin{eqnarray*}
		p_{RB}\frac{\mathsf{SELF}}{d(d+1)\log_2{k}}+(1-p_{RB})\frac{\mathsf{OTHER}}{2(d+1)} & = & \frac{\mathsf{SELF} + \mathsf{OTHER}}{d(d+1)\log_2{k}+2(d+1)}\\
		& \geq & \frac{W^*}{d(d+1)\log_2{k}+2(d+1)},
	\end{eqnarray*}
\end{comment}
	\begin{eqnarray*}
		p_{RB}\frac{\mathsf{SELF}}{2\log_2{k}}+(1-p_{RB})\frac{\mathsf{OTHER}}{4} & = & \frac{\mathsf{SELF} + \mathsf{OTHER}}{2\log_2{k}+4}\\
		& \geq & \frac{W^*}{2\log_2{k}+4},
	\end{eqnarray*}
	as desired.
	
\end{proof}

